Best of Both Worlds: Practical and Theoretically Optimal Submodular Maximization in Parallel

For the problem of maximizing a monotone, submodular function with respect to a cardinality constraint $k$ on a ground set of size $n$, we provide an algorithm that achieves the state-of-the-art in both its empirical performance and its theoretical properties, in terms of adaptive complexity, query complexity, and approximation ratio; that is, it obtains, with high probability, query complexity of $O(n)$ in expectation, adaptivity of $O(\log(n))$, and approximation ratio of nearly $1-1/e$. The main algorithm is assembled from two components which may be of independent interest. The first component of our algorithm, LINEARSEQ, is useful as a preprocessing algorithm to improve the query complexity of many algorithms. Moreover, a variant of LINEARSEQ is shown to have adaptive complexity of $O( \log (n / k) )$ which is smaller than that of any previous algorithm in the literature. The second component is a parallelizable thresholding procedure THRESHOLDSEQ for adding elements with gain above a constant threshold. Finally, we demonstrate that our main algorithm empirically outperforms, in terms of runtime, adaptive rounds, total queries, and objective values, the previous state-of-the-art algorithm FAST in a comprehensive evaluation with six submodular objective functions.

==> FastExp1.tex <==
\subsection{Comparison vs adaptive algorithms from \citet{Fahrbach2018}}

\begin{figure}[t]
  \subfigure[]{
    \includegraphics[width=0.23\textwidth, height=0.11\textheight]{figs/FAST_val-WS_exp1.pdf}\label{fig:SODA_objA}
  }
  \subfigure[]{
    \includegraphics[width=0.23\textwidth, height=0.11\textheight]{figs/FAST_val-CAROAD_exp1.pdf}
  }
  \subfigure[]{
    \includegraphics[width=0.23\textwidth, height=0.11\textheight]{figs/FAST_val-INFMAXCalTech_exp1.pdf} \label{fig:objF}
  }
  \subfigure[]{
    \includegraphics[width=0.23\textwidth, height=0.11\textheight]{figs/FAST_val-MOVIECOVERsubset_exp1.pdf}\label{fig:SODA_objD}
  }
  \subfigure[]{
    \includegraphics[width=0.23\textwidth, height=0.11\textheight]{figs/FAST_query-WS_exp1.pdf}\label{fig:SODA_qryA}
  }
  \subfigure[]{
    \includegraphics[width=0.23\textwidth, height=0.11\textheight]{figs/FAST_query-CAROAD_exp1.pdf}
  }
  \subfigure[]{
    \includegraphics[width=0.23\textwidth, height=0.11\textheight]{figs/FAST_query-INFMAXCalTech_exp1.pdf} \label{fig:objF}
  }
  \subfigure[]{
    \includegraphics[width=0.23\textwidth, height=0.11\textheight]{figs/FAST_query-MOVIECOVERsubset_exp1.pdf}\label{fig:SODA_qryD}
  }
  \subfigure[]{
    \includegraphics[width=0.23\textwidth, height=0.11\textheight]{figs/FAST_time-WS_exp1.pdf}\label{fig:SODA_timeA}
  }
  \subfigure[]{
    \includegraphics[width=0.23\textwidth, height=0.11\textheight]{figs/FAST_time-CAROAD_exp1.pdf}
  }
  \subfigure[]{
    \includegraphics[width=0.23\textwidth, height=0.11\textheight]{figs/FAST_time-INFMAXCalTech_exp1.pdf} \label{fig:objF}
  }
  \subfigure[]{
    \includegraphics[width=0.23\textwidth, height=0.11\textheight]{figs/FAST_time-MOVIECOVERsubset_exp1.pdf}\label{fig:SODA_timeD}
  }
  \caption{Evaluation of adaptive algorithms from \citet{Fahrbach2018} on MaxCover(WS), TrafficMonitor, InfluenceMax and MovieRecommendation in terms of objective value normalized by the standard greedy value (Figure \ref{fig:SODA_objA} -  \ref{fig:SODA_objD}), total number of queries (Figure \ref{fig:SODA_qryA} -  \ref{fig:SODA_qryD}) and the time required by each algorithm (Figure \ref{fig:SODA_timeA} -  \ref{fig:SODA_timeD})} \label{fig:query}
\end{figure} 

 Since \exm and the \bsm algorithm of \citet{Fahrbach2018} has better theoretical guarantee than \fast, we ran additional experiments comparing against both the \exm and the \bsm algorithm, as implemented by the authors of \fast. In this highly optimized implementation, a single query per processor is used in each adaptive round instead of the number of queries required theoretically as description of the implementation in \citet{Breuer2019}. The evaluation was performed on MaxCover(WS), TrafficMonitor, InfluenceMax and MovieRecommendation in terms of objective value normalized by the standard greedy value (Figure \ref{fig:SODA_objA} -  \ref{fig:SODA_objD}), total number of queries (Figure \ref{fig:SODA_qryA} -  \ref{fig:SODA_qryD}) and the time required by each algorithm. In summary, our algorithm \flsabr is faster by roughly an order of magnitude and uses roughly an order of magnitude fewer queries over \bsm.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{Complete proofs are provided in the Supplementary Material.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}
